An End-To-End Analysis of Deep Learning-Based Remaining Useful Life Algorithms for Satefy-Critical 5G-Enabled IIoT Networks

Remaining Useful Life (RUL) prediction is a critical task that aims to estimate the amount of time until a system fails, where the latter is formed by three main components, that is, the application, communication network, and RUL logic. In this paper, we provide an end-to-end analysis of an entire RUL-based chain. Specifically, we consider a factory floor where Automated Guided Vehicles (AGVs) transport dangerous liquids whose fall may cause injuries to workers. Regarding the communication infrastructure, the AGVs are equipped with 5G User Equipments (UEs) that collect real-time data of their movements and send them to an application server. The RUL logic consists of a Deep Learning (DL)-based pipeline that assesses if there will be liquid falls by analyzing the collected data, and, eventually, sending commands to the AGVs to avoid such a danger. According to this scenario, we performed End-to-End 5G NR-compliant network simulations to study the Round-Trip Time (RTT) as a function of the overall system bandwidth, subcarrier spacing, and modulation order. Then, via real-world experiments, we collect data to train, test and compare 7 DL models and 1 baseline threshold-based algorithm in terms of cost and average advance. Finally, we assess whether or not the RTT provided by four different 5G NR network architectures is compatible with the average advance provided by the best-performing one-Dimensional Convolutional Neural Network (1D-CNN). Numerical results show under which conditions the DL-based approach for RUL estimation matches with the RTT performance provided by different 5G NR network architectures.

==> __old/Old_Sections/Numerical_results_RAN.tex <==
\newpage

\section{5G RAN \ac{RTT} numerical results}

\begin{figure*}[ht]
\begin{minipage}[b]{0.48\linewidth}
\centering
\includegraphics[width=\linewidth]{Pictures/5G RAN e TOTALI/plot_256QAM.png}
\caption{Average \ac{RAN} \ac{RTT} vs. $N$, $B$ and \ac{SCS}. $L = 256$.}
\label{fig:img1}
\end{minipage}
\hspace{0.1cm}
\begin{minipage}[b]{0.48\linewidth}
\centering
\includegraphics[width=\linewidth]{Pictures/5G RAN e TOTALI/plot_different_QAMs.png}
\caption{Seconda immagine}
\label{fig:img2}
\end{minipage}
\end{figure*}

In this section performance of 5G RAN will be studied.

% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{Pictures/5G RAN e TOTALI/RAN_RTT.png}
% \caption{\label{fig:RAN_RTT} 5G RAN RTT}
% \end{figure}

We have tested the system for different amount of \acp{AGV}. It is worth mentioning that each \ac{AGV} can both transmit and receive data. 
In \ref{subsec: Network Architecture} we introduced the \ac{5G NR} configurations that we tested, now we describe them more into details.

\subsection{Slice of Public \ac{RAN} in \ac{FR1}}
We assumed to use 5 MHz of bandwidth for our application. The \ac{SCS} we assumed to use is 30 KHz, one of the values allowed in this frequency band. As we can see in Fig.~\ref{fig:RAN_RTT}, \ac{RTT} goes from around 6 ms for 1 \ac{AGV} to around 27 ms for 50 \acp{AGV}. The growth of \ac{RTT} is approximately steady, and can be explained studying the number of resource blocks and the number of \ac{SU}. The number of \ac{RB} is:
\begin{align}
n_{RB} =& \left\lfloor \frac{B}{12\Delta f} \right\rfloor, \label{n_RB}
\end{align}
where $\Delta f$ is the \ac{SCS}. In this \ac{RAN} configuration we have $B = 5 MHz$ and $\Delta f = 30 KHz$, substituting the values in (\ref{n_RB}), we obtain $n_{RB} = 13$. In one subframe, with \ac{SPS} = 30~KHz, there are 28 \ac{OFDM} symbols. Since $T_{ISRP}$, since we are using mini-slots composed by 7 \ac{OFDM} symbols, and since we use 4 mini-slots for the control plane, during each iteration we have 4 \ac{SU} for the data plane. Since 90\% of resources are used for the uplink, we use 3 \ac{SU} for the uplink and 1 \ac{SU} for the downlink, and considering $n_{RB} = 13$, we have \red{up to} 39 \ac{PUSCH} messages and 13 \ac{PDSCH} messages in each $T_{ISRP}$. Assuming to have modulation order equal to 256, that means that each symbol carried by each \ac{OFDM} subcarrier carries 8 bits (1 byte), each \ac{PUSCH} and each \ac{PDSCH} carries 48 bytes. In uplink, each \ac{UE} transmit 32 bytes, that corresponds to a \ac{PDU}-\red{data block} of 104 bytes considering overhead introduced from upper layers of 5G: this means that 3 \acp{PUSCH} are needed for each packet sent, and since there are 39 \acp{PUSCH}, we can serve up to 13 \acp{AGV} per $T_{ISRP}$ (we have ignored the scheduling policies explained in \ref{subsection:5G scheduler} for the sake of simplicity). Uplink traffic of \acp{AGV} is periodic, but they are randomly initialized: the first uplink packet generation instant is uniformly distributed between 0 and 100 ms, that is the uplink periodicity. Since $T_{ICP} = 2 ms$, in 100 ms there are 50 $T_{ISRP}$, and the probability that an \ac{AGV} uplink communication is initialized in a specific $T_{ISRP}$ is 1/50 = 0.02. The probability that $x$ \acp{AGV} choose the same communication cycle can be modeled with a binomial distribution, where $n$ is the number of \acp{AGV} (we can consider the worst case in which $n = 50$) and $p$ is the probability of success, that means the probability of choosing a specific communication cycle, i.e., $p = 0.02$. The probability that 14 or more \ac{AGV} choose the same communication cycle is almost $7.8 \cdot 10 ^{-13}$, which means that the probability that there are not enough resources in the data plane of a communication cycle for the uplink is negligible.
Assuming the same hypotheses made in the previous case, we can obtain a similar result for the downlink traffic. The downlink packets sent to \acp{AGV} is 1 byte, that corresponds to 73 bytes data blocks: this means that 2 \acp{PDSCH} are needed for each packet sent. In downlink there are available one \ac{SU} and 13 \acp{RB}, which means that we can serve up to 6 \acp{AGV} per communication cycle. Neglecting the distribution of packets in the downlink, and assuming that a downlink packet is generated each time that an uplink packet is received, the probability that 7 or more downlink packets are transmitted in a communication cycle is $6.0 \cdot 10 ^{-5}$. If we consider that there is no one-to-one correspondance between uplink and downlink packet, i.e., the actual probability is even lower, then the probability that there are not enough resources in the data plane of a communication cycle for the downlink is negligible.

The purpose of this analysis is to demonstrate that the data plane resources are no the bottleneck of the system: limitations are due to the control plane.
As explained in \ref{subsection:5G scheduler}, in the simulator for each \ac{UE} two \ac{PUCCH}/\ac{PDCCH} pairs are needed: this means that with $n_{RB} = 13$ we can serve up to 6 \acp{UE} in each $T_{ISRP}$. This is the reason why with 1 and 5 \acp{AGV} we have almost the same \ac{RTT}. With 10 \acp{AGV}, two communication cycles are needed, and this lead to an increase in \ac{RTT}: since we have a transmission in uplink followed by a transmission in downlink, up to 4 communication cycles are needed for the whole communication. The fact that the \ac{RTT} increases by approximately 3 ms (i.e., between 1 and 2 times $T_{ISRP}$) from the case with 5 \acp{AGV} to the case with 10 \acp{AGV} is consistent with the analysis just performed. We can see that \ac{RTT} is almost the same for 20 and 25 \acp{AGV}: this is due to the fact that in both cases 4 communication cycle are needed.

\subsection{Private \ac{RAN} in \ac{FR2}}
We assumed to use 100 MHz of bandwidth for the application. The \ac{SCS} we assumed to us is 120 KHz. As we can see in Fig.~\ref{fig:RAN_RTT}, \ac{RTT} goes from around 5 ms to around 8.5 ms. \ac{RTT} is almost constant from 1 to 30 \acp{AGV}, then there is a step increase with 35 \acp{AGV}, and then again it is constant up to 50 \acp{AGV}. With this \ac{RAN} configuration, $B = 100 MHz$ and $\Delta f = 120 KHz$, substituting the values in (\ref{n_RB}), we obtain $n_{RB} = 69$. As before, the data plane resources are not the bottleneck of the system. In the simulator for each \ac{UE} two \ac{PUCCH}/\ac{PDCCH} pairs are needed: this means that with $n_{RB} = 69$ we can serve up to 34 \acp{UE} per communication cycle. This is the reason why there is a steep increase in \ac{RTT} going from 30 to 35 \agp{AGV}.


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{Pictures/5G RAN e TOTALI/Total_RTT.png}
\caption{\label{fig:Total_RTT} Total RTT}
\end{figure}
===========================


% scusa nico ho dovuto togliere il rosso
% Dubbio: nel simulatore i subframe sono di 2 ms invece che 1 ms come da standard perchè con 1 ms ci venivano 4 SU in un subframe, che sono sufficienti solo per il piano di controllo!

% self.n_su_per_subframe = int(4 * self.subcarrier_spacing / 15)
% riga 74 in centrlized.py


